From Pixels to Personas: Investigating and Modeling Self-Anthropomorphism in Human-Robot Dialogues

Self-anthropomorphism in robots manifests itself through their display of human-like characteristics in dialogue, such as expressing preferences and emotions. Our study systematically analyzes self-anthropomorphic expression within various dialogue datasets, outlining the contrasts between self-anthropomorphic and non-self-anthropomorphic responses in dialogue systems. We show significant differences in these two types of responses and propose transitioning from one type to the other. We also introduce Pix2Persona, a novel dataset aimed at developing ethical and engaging AI systems in various embodiments. This dataset preserves the original dialogues from existing corpora and enhances them with paired responses: self-anthropomorphic and non-self-anthropomorphic for each original bot response. Our work not only uncovers a new category of bot responses that were previously under-explored but also lays the groundwork for future studies about dynamically adjusting self-anthropomorphism levels in AI systems to align with ethical standards and user expectations.

==> figures/amt_nsa2sa.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={12 0 0 0},clip,width=8cm]{figures/amt_nsa2sa.png}
  \caption{AMT survey results on preference for (a) Zoogle Assistant and (b) Jamie the Robot, transitioning from NSA to SA.}
  \label{fig_nsa2sa}
  \vspace{-3mm}
\end{figure}

==> figures/amt_nsa2sa_humanoid.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=7.8cm]{figures/amt_nsa2sa_humanoid.png}
  \caption{nsa2sa}
  \label{fig_nsa2sa_humanoid}
  % \vspace{-3mm}
\end{figure}

==> figures/amt_nsa2sa_zoogle.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=7.8cm]{figures/amt_nsa2sa_zoogle.png}
  \caption{nsa2sa}
  \label{fig_nsa2sa_zoogle}
  \vspace{-3mm}
\end{figure}

==> figures/amt_sa2nsa.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={12 0 0 0},clip,width=8cm]{figures/amt_sa2nsa.png}
  \caption{AMT survey results on preference for (a) Zoogle Assistant and (b) Jamie the Robot, transitioning from SA to NSA.}
  \label{fig_sa2nsa}
  \vspace{-3mm}
\end{figure}

==> figures/amt_sa2nsa_humanoid.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=7.8cm]{figures/amt_sa2nsa_humanoid.png}
  \caption{sa2nsa}
  \label{fig_sa2nsa_humanoid}
  \vspace{-3mm}
\end{figure}

==> figures/amt_sa2nsa_zoogle.tex <==
\begin{figure}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=7.8cm]{figures/amt_sa2nsa_zoogle.png}
  \caption{sa2nsa}
  \label{fig_sa2nsa_zoogle}
  \vspace{-3mm}
\end{figure}

==> figures/amt_screenshot_chatbot.tex <==
\begin{figure*}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=16cm]{figures/amt_screenshot_chatbot.png}
  \caption{Screenshot of the AMT task interface where workers select the more appropriate response for the Zoogle Assistant Chatbot in various dialogue scenarios.}
  \label{fig_amt_screenshot_chatbot}
  % \vspace{-3mm}
\end{figure*}

==> figures/amt_screenshot_humanoid.tex <==
\begin{figure*}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=16cm]{figures/amt_screenshot_humanoid.png}
  \caption{Screenshot of the AMT task interface where workers select the more appropriate response for the Jamie the Robot in various dialogue scenarios.}
  \label{fig_amt_screenshot_humanoid}
  % \vspace{-3mm}
\end{figure*}

==> figures/amt_screenshot_inst.tex <==
\begin{figure*}[htb!]
  \centering
  \includegraphics[trim={0 0 0 0},clip,width=16cm]{figures/amt_screenshot_inst.png}
  \caption{Screenshot of instructions we present to AMT workers.}
  \label{fig_amt_screenshot_inst}
  % \vspace{-3mm}
\end{figure*}
